Guided Linear Upsampling

Guided upsampling is an effective approach for accelerating high-resolution image processing. In this paper, we propose a simple yet effective guided upsampling method. Each pixel in the high-resolution image is represented as a linear interpolation of two low-resolution pixels, whose indices and weights are optimized to minimize the upsampling error. The downsampling can be jointly optimized in order to prevent missing small isolated regions. Our method can be derived from the color line model and local color transformations. Compared to previous methods, our method can better preserve detail effects while suppressing artifacts such as bleeding and blurring. It is efficient, easy to implement, and free of sensitive parameters. We evaluate the proposed method with a wide range of image operators, and show its advantages through quantitative and qualitative analysis. We demonstrate the advantages of our method for both interactive image editing and real-time high-resolution video processing. In particular, for interactive editing, the joint optimization can be precomputed, thus allowing for instant feedback without hardware acceleration.

==> analysis.tex <==
\section{Analysis}
\label{sec:analysis2}

An ideal guided upsampling method should be able to keep the edge shape of the original image while preserving detail effects of the target image, which may be contradictory for some applications such as detail enhancement. In the below we will analyze the ability  our method in these aspects and show its connections with previous methods.

\subsection{Edge Recovery}
\label{sec:connections}

Typical image edges can be classified as three types: step edge, ramp edge, roof edge~\cite{koschan2005detection,yin2019side}. For natural images, most edges should be the ramp edges connecting two regions. Obviously, the transition effects of the ramp edges can be well represented by the linear interpolation of the two region colors. Therefore, by interpolating only two pixels, GLU can recover edges of the original image very well. As a comparison, using GNU can recover only the step edge, and thus would introduce noticeable artifacts.

A natural question is whether we can achieve further improvements by interpolating more pixels? In fact, \refeq{eq:interpT} can be more generally represented as
 \begin{equation}
 	\hat{T}_p=\sum\limits_{q\in\Omegaplow} \omega_q\;\Tlow_q 
 	\label{eq:general}
 \end{equation}
with $\omega_q$ is the normalized weights. Interestingly, this is exactly the form of JBU. However, in JBU $\omega_q$ is not optimized, and the filtering effect would result in blur and edge reversal artifacts~\cite{he2012guided}. It is easy to see that when $\sigma_d\to \infty$ and $\sigma_r\to 0$, JBU will reduce to GNU. In practice by decreasing $\sigma_r$, the blur artifacts of JBU can be alleviated, but it is still hard to recover edges as well as GLU. 

%In GLU, good results can be achieved by the weighted average of only 2 low-resolution pixels. This is mainly because most edges of natural images are the ramp edges~\cite{yin2019side} as shown in \reffig{fig:edges}. The ramp edges are the transitions between two regions with different color, and thus can be well approximated by the linear interpolation of the two region colors. 

Although we have not tested, we argue that it is unnecessary to take more pixels for the interpolation. Involving more pixels not only make the optimization more difficult, but also may lead to overfitting and extrapolation, both will reduce the result quality of the target image. 

The roof edge is easy to be lost by the downsampling, as we have demonstrated in \reffig{fig:downsample}. The proposed downsampling optimization method is helpful to alleviate this problem. However, for large ratio of downsampling it is still inevitable, as we will demonstrate in section \ref{limitation}.

\subsection{Detail Preservation}
\label{sec:details}

The connection of our method with previous local color transformation methods~\cite{he2012guided,chen2016bilateral} has been revealed in section \ref{sec:derivation}. Although our method also implicitly takes advantage the local color transformation for transferring the upsampling parameters, it should be noted that unlike the \emph{guided filter} and BGU, our method does not require the transformations to be smooth in either the image space or the bilateral space. Therefore, it can better preserve detail effects of the target image, as shown in \reffig{fig:downsample}. 

One may concern that the lacking of smooth constraint would introduce artifacts. Although keeping smoothness is important for most image processing operators, we find that our method with each pixel independently solved also works well in most situations. This is mainly because the linear interpolation model can well approximate the appearance of the original image, which serves as a smooth guidance map that can suspend unsmooth artifacts. However, for the case that the pixel affinities of the source and the targe images are significantly different, artifacts may be produced for the target output (see section \ref{limitation} for examples).

%Since our method operates in pixel level, it can be suited for more general cases than previous methods based on the color line model and local color transformation. On one hand, multiple color lines in a local patch can be represented with our method because each pixel takes its own color line. On the other hand, 

%In addition, since in our method each pixel takes an individual color line, it can deal with more general case that there exists multiple color lines locally.

\begin{figure}[t]   
	\centering
	\includegraphics[width=\linewidth]{edge.pdf}
	\caption{Models of three ideal edges. (a) Step edge (b) Ramp edge  (c) Roof edge.}
	\label{fig:edges}
\end{figure}

\begin{figure}[t] 
  \centering 
  \subfigure[Input image]{
    \includegraphics[width=0.235\columnwidth]{figure/fig7/input.png}
    } \hspace{-2.5mm}
    \subfigure[Ground truth]{
    \includegraphics[width=0.235\columnwidth]{figure/fig7/gt.png}
    } \hspace{-2.5mm}
  \subfigure[BGU]{ 
    \includegraphics[width=0.235\columnwidth]{figure/fig7/bgu.png}
    }\hspace{-2.5mm}
  \subfigure[GLU]{
    \includegraphics[width=0.235\columnwidth]{figure/fig7/glu.png} 
    } 
  \caption{(a) Input an $8\times$ downsampled matted image, guided by original image. Upsampled ground truth shown as (b). (c) BGU tends for bleeding effects among foreground and background. (d) Proposed GLU is superior in detail preserving.}
  \label{fig:bleeding}
\end{figure}



\begin{comment}
\subsection{Edge Recovery}
Challenges of upsampling technology are that the edges are easily blurred and the image details are difficult to renovate during the enlargement process.
The edge of a natural image is the discontinuity of the local features of the image, and we define the boundary of the region where the grayscale changes sharply in the image as the edge. The edge can be regarded as the fusion of two images. According to the effect of fusion, that is, the intensity of the grayscale change, the edge is usually divided into step edge, ramp edge, and roof edge. We model them in 2D signal space as shown in Figure.\ref{fig:edges}. 

Among these three edges, (a) and (b) are essentially the same type, but the degree of ambiguity of the two is different. We could consider edge(b) as a Gaussian blur of edge(a). Based on reality, edge(b) is the most common type in natural images. And as for edge c, it is a great challenge for restoration in upsampling, for numerous details will be lost during downsampling. Optimized downsampling technique provided in Sec. \ref{sec:3.3} preserves details better, making it possible to reconstruct fine edges. 

Focusing on the three types of edges in natural image, guided by original high-resolution image, given its thumbnail, we compare the ability of reconstructing original image between our proposal with alternative upsampling methods. As shown in Figure.\ref{fig:compare}, testing nature image with typical edges(b) and (c) in Figure.\ref{fig:edges} are shot, we take 1/8 reduced image as input Figure.\ref{fig:compare}(a), and we demonstrate an objective upsampling comparison of edges reconstruction with other algorithms. 
Among them, Figure.\ref{fig:compare}(d) demonstrates optimal nearest neighbor upsampling, rather than a pair of optimal sampling points mentioned in \ref{sec:3.2}, the closest point to $p^{'}$ and another optimal sampling point are selected, and exploited by the same upsampling strategy eq. \ref{eq:4}. And Figure.\ref{fig:compare}(e) is our optical linear upsampling method. 
Notably, our upsampling proposal is free of target image, i.e. optimization upsampling parameters will not vary in changes of target image, unlike the output-dependent guided upsampling algorithms. Our proposal is more suitable for situations where output changes throughout, such as user interactively modifying on target image. Joint bilateral upsampling \cite{kopf2007joint} also has the same advantages, but their approach are prone to oscillation or blurring at the edges, results in piece-wise smooth images, while our method can generate satisfactory results. %In particular, with proposed optimized downsampling method, our technique can reconstruct fine edges. 
	
\end{comment}
	





